More is Less: Perfectly Secure Oblivious Algorithms in the Multi-Server Setting

The problem of Oblivious RAM (ORAM) has traditionally been studied in a single-server setting, but more recently the multi-server setting has also been considered. Yet it is still unclear whether the multi-server setting has any inherent advantages, e.g., whether the multi-server setting can be used to achieve stronger security goals or provably better efficiency than is possible in the single-server case. In this work, we construct a perfectly secure 3-server ORAM scheme that outperforms the best known single-server scheme by a logarithmic factor. In the process, we also show, for the first time, that there exist specific algorithms for which multiple servers can overcome known lower bounds in the single-server setting.

==> conclude.tex <==
\section{Conclusion and Open Questions}
Oblivious RAM and oblivious algorithms 
in the multi-server setting 
are in general less understood than in the single-server
setting.

\elaine{write some open questions}


==> defn-antigoni.tex <==
% !TEX root =./multiserver.tex

\section{Definitions}
\subsection{RAM Model of Computation}

The RAM model consists of a CPU and a memory storage of size $M$. The CPU executes a program that can access the memory by using read/write operations. In particular, for a program $P$ with memory of size $\memsz$ we denote the initial contents of the memory data by $D \in \mathbb{Z}_q^\memsz$ where $q \in \N$ is the size of the word. Additionally, the program gets a ``short'' input $x \in \mathbb{Z}_q^\inpsz$, which we alternatively think of as the initial state of the program.

We use the notation $P^D(x)$ to denote the execution of program $P$ with initial memory contents $D$ and input $x$. The program $P$ can read from and write to various locations in memory $D$ throughout its execution.

We will also consider the case where several different programs are executed sequentially and the memory persists between executions. We denote this process as $(y_1, \ldots, y_\ell) = (P_1(x_1),\ldots,P_\ell(x_\ell))^D$ to indicate that first $P_1^D(x_1)$ is executed, resulting in some memory contents $D_1$ and output $y_1$, then $P_2^{D_1}(x_2)$ is executed resulting in some memory contents $D_2$ and output $y_2$ etc. As an example, imagine that $D$ is a huge database and the programs $P_i$ are database queries that can  read and possibly write to the database and are parameterized by some values $x_i$.


\paragraph{CPU-Step Circuit.} Consider an execution of a RAM program which involves at most $T$ $\CPU$ steps. We represent a RAM program $P$ via a small \emph{$\CPU$-Step Circuit} which executes a sequence of $T$ $\CPU$ steps. In this work we will denote one CPU step by:
$$C^P_{\CPU}(\state,\md) = (\state',\RorW,L,z)$$
%$$C^P_{\CPU}(\state, z^{\read}) = (\state', L, z^{\wrt}).$$
This circuit takes as input the current CPU state $\state$ and a block $\md$. Looking ahead the block $\md$ will be read from the memory location that was requested in the previous $\CPU$ step. The $\CPU$ step outputs an updated state $\state'$, a read or write bit $\RorW$, the next location to read/write $L \in [\memsz]$, and a block $z$ to write into that location ($z=\bot$ when reading).  The sequence of locations and read/write values collectively form what is known as the \emph{access pattern}, namely $\sf{MemAccess}=  \{L^{\step}  : \step = 1,\ldots,T\}$.

\paragraph{Representing RAM computation by CPU-Step Circuits.} The computation $P^D(x)$ starts with the initial state set as $\state_0 = x$ and initial read location $L^0=0$ as a dummy read operation. In each step $\step \in \{0,\ldots T-1\}$, the computation proceeds by first reading memory location $L^{\step}$, that is by setting $\md^{\step} := D[L^{\step}]$ if $\step \in \{1,\ldots T-1\}$ and as $0$ if $\step=0$.  Next it executes the CPU-Step Circuit $C^P_{\CPU}(\state^{\step}, \md^{\step}) = (\state^{\step+1}, L^{\step+1}, z^{\step+1})$. Finally if $z^{\step+1}\neq \bot$ we write to the location $L^{\step}$ by setting $D[L^{\step}] := z^{\step+1}$. If $\step = T-1$ then we set $\state$ to be the output of the program $P$ and ignore the value $L^{\step+1}$. Note here that we have without loss of generality assumed that in one step of the CPU-Step circuit the same location in memory is read from and written to. This has been done for the sake of simplifying exposition.
\anti{need to shorten the above description}



\begin{definition} [$\kappa$-server model]
The $\kappa$-\emph{server model} is defined by a client $C$ interacting with $\kappa$ servers $\{ S_i \}_{i \in [\kappa]}$.
$C$ is modelled as an interactive machine with bounded (constant) sized memory. 
\end{definition}

We will realize the following functionality. 

\protocoll{\textbf{Functionality $F_f$}}
{$\kappa$-Server functionality.}{fig:funct}{
$F$ runs with servers $S = \{S_1,\ldots, S_\kappa\}$ and an
adversary $\mathcal{S}$ who corrupts a subset $I \subset [\kappa-1]$ of servers.
\begin{enumerate}
\item For each $i \in [\kappa]$, the functionality receives $x_i$
from server $S_i$.

\item Upon receiving the inputs from all servers, evaluate the function $(y_1,\ldots y_\kappa)=f(x_1,\ldots x_\kappa;\rho)$ and
 send $y_1,\ldots y_\kappa$ to $\mathcal{S}$.

\item Upon receiving ${\sf deliver}$ from $\mathcal{S}$,
the functionality sends $y_1,\ldots y_\kappa$ to all parties.
\end{enumerate}}



%Before we formally define our $\kappa$-\emph{server ORAM} we extend our notation to work for $\kappa$ servers. 

\begin{definition} [$\kappa$-Server Oblivious RAM]\label{d:ost} An oblivious $\kappa$-Server $\ORAM$ scheme consists of procedures $(\OData, \OProg)$ with syntax:
\begin{itemize}

\item $\oD \gets \OData(1^\secp,1^\kappa,D)$: Given a security parameter $1^\secp$, memory data $D\in \mathbb{Z}_q^\memsz$, outputs oblivious memory $\oD\in \mathbb{Z}_q^{\kappa \times \omemsz}$. The polynomial-time algorithm $\sf Map$ generates $\oD$ as follows: 
\begin{itemize}
\item A $\kappa$-\emph{server Memory Mapping} $\sf Map$ on input a memory word $u \in \mathbb{Z}_q$ in the $i^{th}$ memory location, expands it to a $\kappa$-dimensional vector, i.e., ${\sf Map}(u)=(u_1,\dots, u_k) \in \mathbb{Z}_{q}^{\kappa}$. For all $i\in[\kappa]$, $u_i$ is stored in $\oD_i$. The  polynomial-time algorithm $\sf IMap$ on input $\kappa$ elements $u_1, \ldots, u_k \in \mathbb{Z}_q$ reconstructs $u \in \mathbb{Z}_q$.\\
The oblivious memory  $\oD$ consists of all the $\kappa$ memories $\oD_1,\ldots, \oD_\kappa$ such that $\oD \in \mathbb{Z}_q^{\kappa\times \omemsz}$. 

\end{itemize}


\anti{there is an issue here since not all the servers store secret share versions of the data}

\item $\oP \gets \OProg(1^\secp,1^\tcur,P)$: On input a security parameter $1^\secp$ and a program $P$ with running time $T$, outputs an oblivious program $\oP$ which works over the encoded data $\oD$.




\end{itemize}
\end{definition}


For any data $D$, programs $P_1, \ldots, P_\ell$ with polynomially-bounded run-times $T_1,\ldots,T_\ell$ and all inputs $x_1,\ldots,x_\ell$ consider the experiment of selecting $\oD \gets \OData(1^\secp,D), {\oP_{i}:= \OProg(1^\secp,1^{\tcur_i},P_i)}$. Then we require the following:
\paragraph{Correctness.} $\Pr[(\oP_1(x_1),\ldots,\oP_\ell(x_\ell))^{\oD}= (P_1(x_1),\ldots,P_\ell(x_\ell))^D]=1$.


\paragraph{Obliviousness.}   For an oblivious $\ORAM$ scheme, we require that there exists
an unbounded simulator $\SimORAM$, such that for any polynomial-length sequence of memory access $\MemAccess_D$ on data $D$
$$({\oD},\OMemAccess_{\oD} )\equiv \SimORAM(g(\MemAccess_D),\{T_i\}_{i\in[\ell]}) $$

where $\OMemAccess_{\oD}$ is the physical addresses generated by the $\ORAM$ scheme during a sequence of operations $\MemAccess_D$ for the execution $(\oP_1(x_1),\ldots,\oP_\ell(x_\ell))^{\oD}$ and $g(\MemAccess_D)$ is referred to as the leakage function. 

%\paragraph{Perfect secrecy.}  Let $\oD \in \mathbb{Z}_q^{\kappa \times \omemsz}$  be the oblivious memory consisting of all the $\kappa$ memories. For every $j\in[n]$ and every set $S\subseteq [k]$ such that $|S|=t$ the values $\{M'[i,j]\}_{i \in [k]\setminus S}$ are distributed uniformly at random.  
   
 



\paragraph{Efficiency.}  \anti{to do}






